Virtual element method for the system of time dependent nonlinear convection-diffusion-reaction equation

In this work, we have discretized a system of time-dependent nonlinear convection-diffusion-reaction equations with the virtual element method over the spatial domain and the Euler method for the temporal interval. For the nonlinear fully-discrete scheme, we prove the existence and uniqueness of the solution with Brouwer's fixed point theorem. To overcome the complexity of solving a nonlinear discrete system, we define an equivalent linear system of equations. A priori error estimate showing optimal order of convergence with respect to $H^1$ semi-norm was derived. Further, to solve the discrete system of equations, we propose an iteration method and a two-grid method. In the numerical section, the experimental results validate our theoretical estimates and point out the better performance of the two-grid method over the iteration method.

==> meshdata.tex <==
%\documentclass[10pt,a4paper]{article}
%\usepackage[latin1]{inputenc}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
%\usepackage{graphicx}
%\begin{document}

	
\begin{table}[h]
\centering % centering table
\begin{tabular}{|c c c | c c c | c c c|} % creating 10 columns
\hline % inserting double-line
\multicolumn{3}{|c|}{hexagon} & \multicolumn{3}{|c|}{nonconvex} & \multicolumn{3}{|c|}{random voronoi} \\
\hline % inserts single-line
$h$ & dof & $N_E$ & $h$ & dof & $N_E$ & $h$ & dof & $N_E$ \\ %\hline
0.0436&3323&1660&0.0442&4801&1600&0.0405&10655&5700 \\
0.0219&13042&6520&0.0221&19201&6400&0.0213&42709&23000 \\ 
0.0115&51682&25840&0.0110&76801&25600&0.0113&150617&81800\\ 
0.0055&205762&102880&0.0054&307201&102400&0.0054&632372&340000 \\ \hline
\end{tabular}
\caption{Mesh parameters with degrees of freedom (dof) and number of elements ($N_E$).} % title name of the table
\label{tab:mesh}
\end{table}

%\end{document}
